LUMINOUS: Indoor Scene Generation for Embodied AI Challenges

Learning-based methods for training embodied agents typically require a large number of high-quality scenes that contain realistic layouts and support meaningful interactions. However, current simulators for Embodied AI (EAI) challenges only provide simulated indoor scenes with a limited number of layouts. This paper presents Luminous, the first research framework that employs state-of-the-art indoor scene synthesis algorithms to generate large-scale simulated scenes for Embodied AI challenges. Further, we automatically and quantitatively evaluate the quality of generated indoor scenes via their ability to support complex household tasks. Luminous incorporates a novel scene generation algorithm (Constrained Stochastic Scene Generation (CSSG)), which achieves competitive performance with human-designed scenes. Within Luminous, the EAI task executor, task instruction generation module, and video rendering toolkit can collectively generate a massive multimodal dataset of new scenes for the training and evaluation of Embodied AI agents. Extensive experimental results demonstrate the effectiveness of the data generated by Luminous, enabling the comprehensive assessment of embodied agents on generalization and robustness.

==> article/framework.tex <==
\section{Luminous(Obsolate)}
\subsection{Framework overview}
\begin{figure}
    \centering
    \includegraphics[width=0.9\textwidth]{./images/framework_luminous.pdf}
    \caption{The Luminous Framework.}
    \label{fig:framework}
\end{figure}

We apply state-of-the-art methods for indoor scene generation that focus on generating meshes represented by object types, positions, rotations and scales. Then the indoor scene fulled mesh information helps the downstream tasks such as generating point clouds or voxels~\cite{roldao20213d}. Methods included in Luminous are not only deep-learning based~\cite{wang2020sceneformer, wang2019planit}, but energy-based~\cite{qi2018human} or rule-based~\cite{ma2018language}. Our motivation is to apply all of collected algorithms to generate indoor scenes by the same settings w.r.t. room structures, object and texture pools, light settings and e.t.c.

We re-implemented some of the algorithms since some the them are missing data or Python code. The scene generation parts are applied to synthesis scenes from the same set of \textit{raw materials} obtained from some public datasets (e.g. 3D-FRONT~\cite{fu20203d}) and toolboxes (e.g. \thor~\cite{kolve2017ai2}).

The qualify of synthesized scenes are accessed by the automatic evaluation metrics provided by Luminous. We also provide pipelines that are connected to Amazon Mechanical Turk (MTurk) with detailed designs for user studies.

To facilitate researches in Embodied AI, we integrate those methods with game development by Unity, and 3D creation by Blender.

\subsection{Architecture}
As we shown in Figure \ref{fig:framework},  the overall structure of \framework{}  mainly consists of three components. First, we propose a unified representation of indoor scene processing, providing various interfaces for data processing, making the original data in different formats required by different models: e.g. RGB images, bounding boxes with object types, etc. After that, different data formats are used as inputs to different models for training indoor scene generation models. It is worth noting that we unify the model-generated scene formats again, allowing us to use the same scene rendering tools to automatically visualize the scenes. Finally, we provide different testing interfaces to uniformly evaluate the quality of various algorithm-generated scenarios.

\textbf{Data processing}\\
Since our ultimate task is to provide indoor scenes as experimental environments for Embodied AI, the data we target should provide a full set of information about the indoor scenes: e.g., house structure, furniture models, and object placement information. Luminous  selects three data sources for data processing: mesh information from SUNCG~\cite{song2017semantic}, mesh information from 3D-FRONT~\cite{fu20203d}, and game designs from \thor~\cite{kolve2017ai2}. In the data processing, we first unify the names of items in different datasets (e.g.  \textit{picture} $=$ \textit{painting}, \textit{bedside cabinet} $=$ \textit{nightstand}). The full list of unified furniture and object names are attached in the appendix. Then we normalize the coordinated w.r.t. locations and rotations. We also normalize room scales. Finally, according to different formats of the training data for different methods, we generally provides three different data formats: RGB-D images, semantic segmentation, and bounding boxes together with object types and rotations. 

\textbf{Scene Synthesis}\\
Luminous provides some state-of-the-art algorithms for indoor scene synthesis. We chose Python as programming language ,and Pytorch  for deep learning. We have carefully referred to the source code of these these methods. However, for the reason such as missing public training dataset, and the compromise we have made for unifying data formats (e.g. \textit{double bed} $\to$ \textit{bed}), the re-implemented performance in Luminous for those methods may differ from the original one. The details of the re-implementation will be discussed in the Appendix.

\textbf{Rendering}\\
% We provide interfaces for indoor scene rendering based on two open source tools: Blender and AI2THOR. Blender is a free and open-source 3D computer graphics tool that can bring the synthesized indoor scenes into other 3D applications such as 3D animations and 3D printings. AI2THOR, an interactable framework for Embodied AI agents based on Unity,  can bring the indoor designs into game development and researches for Embodied AI. After getting the unified format of scene outputs including the category and location information, we render the scenes according to the following rules:
% \begin{itemize}
%     \item If the generative model does not specifically predict the house structure, we assume that the room is a rectangle with a length-width-height of $1:1:0.6$.
%     \item If the model does not have a description of the furniture mesh details (e.g. color and material), then we pick a random one of that type from the furniture library and adjust it to the specified size. 
%     \item Since our framework is for Embodied AI, we want the original scene where agents are located be collision-free. If there are items overlapping in the generated scene, we fine-tune the item positions by random shifting until there is no collision.
% \end{itemize}
The propose of our rendering process is to ensure that scenes generated by different models are consistent with respect to style, lighting, resolution, etc.

\textbf{Evaluation}\\
We refer to the evaluation methods applied by different methods, and propose three categories of criteria to evaluate the quality of synthesized indoor scenes: quantitative metrics to compare the original scenes in the training dataset with synthesized ones, user studies performed on the synthesized scenes, and Embodied AI metrics to evaluate the potential of the synthesized scenes to support Embodied AI studies. We refer to the details in the Appendix.

\subsection{Constrained Stochastic Scene Generation}
We consider the problem of indoor scene generation under certain constraints represented by text descriptions~\cite{ma2018language} or scene graphs~\cite{luo2020end}. In our baseline, each constraint not only defines the type of an object, but also optionally describes the object's relationship with others in the scene. In detail, a constraint $c_i$ provides the information for placing object $i$ by defining its type $o_i$ (e.g. \textit{bed}), and a set of relationship with others $R_i = \{ rel(i, j_k))\}_{k=1,2,...}$, where $j_k$ stands for another object in the scene and $rel(\cdot, \cdot)$ specifies the relationship between two objects (e.g. \textit{bed} \textit{\textbf{beside}} \textit{window}).

Given a set of constraints $\{c_i\}_{i=1,2,...}$ and the room structure (the shape of floor, wall and ceiling), an indoor scene is sampled from a sequential process of three layers. The first layer samples pieces of \textbf{furniture} that represent the overall function of the room and can be placed directly on the floor, such as \textit{bed, dinning table}, and \textit{refrigerator}. The second layer samples \textbf{objects} that are usually supported by another piece furniture such as \textit{book, pen}, and \textit{coffee machine}. Finally, the third layer samples \textbf{decorations} in the scene such as \textit{painting} and \textit{carpet}.

In each layer, we empirically defined the priority value $q(i)$ as the order for placing furniture according to object types. For example, we prefer to place \textit{desk} before placing \textit{chair}: $q(desk) > q(chair)$. Besides, we limit the constraints that can be represented by a direct acyclic graph (DAG) and resolve the relationship between objects to ensure that when calculating $rel(i, j_k)$, we have $q(i) > q(j_k)$. For example, if the text description says \textit{a desk is in front of a chair}, it is resolved as \textit{a chair faces a desk}. %and the original constraints are $(chair, \emptyset) \cup (desk, (chair, in~front~of))$, the the re-calculated constraint become $(desk, \emptyset) \cup (chair, (desk, face))$.

When placing each object, we samples the position and rotation of the object by its explicit relationship with others $\{ rel(i, j_k))\}_{k=1,2,...}$ defined previously, and implicit relationship with others $\{ \widetilde{rel}(i, j_k))\}_{k=1,2,...}$  predefined heuristically from our prior knowledge. For example, Feng Shui usually would come out strongly in favor of pushing the \textit{bed} up against the \textit{wall} of a \bedroom\ $(bed, (wall, against))$. 

Each relationship $rel(i,j_k)$ generates a vector field in space: each position $p$ is characterized by $(s_{p,k}, r_{p,k})$, where $s_{p,k}$ is the score of the point. $s_i$ depends on the distance $d_i$ between $p$ and the target object $j_k$. Figure \label{???}(a) shows different types of relationship and the scores deduced by the relative distance. $r_{p,k}$, suggesting the relative rotation of placing the object, depends on the direction vector from $p$ to its target $j_k$ the type of relationship. Combining $s_{p,k}$ with parameter $w_{type(rel(i,j_{k}))}$ related only the type of relationship, we sample the position to place object $i$ according to weighed sum of scores among all relationship, and the rotation of the object at position $p$ is defined by the type of relationship which has the largest weight.
\begin{align}
    s_p &= \sum_{k} w_{type(rel(i,j_{k}))}\\
    P(p | R_i) &\propto \exp(-s_p) \\
    r_{p} &= r_{p,k'}   ~~~~k' = \arg\max \{w_{type(rel(i,j_{k}))}\}
\end{align}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\textwidth]{images/baseline_sampling.pdf}
    \caption{Illustration of how to sample the position of an object according to the type of relationship. (a) Score functions for different types of relationship, depended on the distance between the sampling position $p$ and the target object $j_k$. (b) Direction vectors suggesting the rotation $r_{p,k}$ of the object being placed on the position.}
    \label{fig:my_label}
\end{figure}
We encourage readers to refer to Appendix ??? where we list 





 

% We follow the formulation in \cite{qi2018human} to represent an indoor scene: an attributed S-AOG~\cite{mumford2007stochastic}. An attributed S-AOG is a probabilistic grammar model with attributes on the terminal nodes. It combines a probabilistic context free grammar (PCFG), and contextual relations. %The structure of S-AOG is shown in Figure ???.  
% Instead of representing contextual relations between furniture as a conditional random field, we perform an simpler rule-based approach to represent them. 



% \begin{figure}
%     \centering
%     \includegraphics[width=.8\textwidth]{images/baseline_aog.pdf}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

% In detail, the S-AOG samples indoor scenes by a top-down grammar. First, we samples the room structure according to the room type (e.g. bedroom). Afterwards the large pieces of furniture in the room are sampled (e.g. bed). Then, we sample small objects that could be on the placed on another piece of furniture (e.g. cellphone). Finally, some decorations are added to the scene to further furnish the room. 

%
\begin{figure}
    \centering
    \includegraphics[width= \textwidth]{images/baseline_example.pdf}
    \caption{Generated indoor scenes from our baseline. All scenes shown are generated under the same constraints (encoded in a scene graph). The blue arrow suggests a piece of furniture is \textit{beside} some place, and the yellow arrow suggests an object is \textit{supported} by some furniture.}
    \label{fig:my_label}
\end{figure}


\subsection{Benchmarking state of the art}
% \lkxcom{this part is not related work section, we should emphasize the different outputs/inputs of those methods and how does these different outputs integrated in \framework{}}
We re-implement several state-of-the-art methods for indoor scene synthesis in Luminous.

\textbf{Deep Priors}~\cite{wang2018deep} represents 3D scenes with orthographic top-down views and learns convolutional neural networks to predict the completion status of the scene, the category of object to add next, and the location to put the object.Each time this model makes a prediction, our re-trained model will first determine whether the indoor scene is complete or not. After that, it completes the incomplete scenes. Our retrained model outputs the predictions based on the furniture model in 3D-FRONT, and outputs the desired items of the scene with their coordinates and rotations.

\textbf{Fast \& Flexible}~\cite{ritchie2019fast}, another deep convolutional generative models, operates on top-down image-based representations, and samples objects iteratively into the scene by predicting their category, location, orientation and size with separate neural network modules. Our retrained model predicts the types, coordinates, rotations and sizes of the items according to the original model, in turn, based on the existing scenes.

\textbf{Human-centric Indoor Scene Synthesis}~\cite{qi2018human} applies a probabilistic grammar model together with a human-centric method to sample and synthesize 3D room layouts. The contextual relations between objects are encoded by Markov Random Fields (MRF). It learns the distributions from an indoor scene dataset and sample new layouts using Markov Chain Monte Carlo (MCMC).  Our framework does not train the model, but directly transforms the original model predictions. The original prediction results show the layout of the indoor scene with rectangular bounding boxes labeled with the location and size of the items. We determine the rotation of the items according to the empirical rules of our baseline.

\textbf{3D-SLN}~\cite{luo2020end} proposes an end-to-end variational generative model
for scene layout synthesis conditioned on scene graphs. Their essential idea is that a 3D scene is represented by an abstract but general scene
graph that helps the synthesis of diverse scene layouts that satisfy relationships included, which provides more flexibility in the synthesis process. For this model, we also re-train on the 3D-FRONT dataset. Since the setup of the method is similar to the baseline: the scene is generated according to the scene graph, we directly render the generated scene of the model without much modification.

==> article/framework_new.tex <==
\section{Luminous}
\subsection{Framework overview}
\framework\ aims to bridge the field of indoor scene generation and Embodied AI tasks. First, Luminous is able to apply the scenes generated by the indoor scene generation model to the Embodied AI simulator. In order to do this, we designed a uniform indoor scene format (CDF), a concise and document conforming to human descriptions to store information about the various objects in the indoor scene. Second, the framework provides an interface to generate Embodied AI training data, mainly including language-based navigation and interaction. In addition, we also use the framework as a platform for Embodied AI model testing: random scenes generated by the models are used to test the performance of different models in more diverse scenarios.

\subsection{Database}
\framework  selects two large-scale synthesized datasets: SUNCG~\cite{song2017semantic} and 3D-FRONT~\cite{fu20203d}, and one set of human-designed scenes \thor~\cite{kolve2017ai2} as resources for indoor scenes. \framework  unifies item names in different datasets (e.g.  \textit{picture} $=$ \textit{painting}, \textit{bedside cabinet} $=$ \textit{nightstand}), normalizes coordinates for locations, rotations and room scales, and provides CDF as the unified scene design files to represent scenes. The full list of unified furniture and object names are attached in the appendix. Besides, \framework applies \thor\ [???], an interactable framework for Embodied AI agents based on Unity, to hold indoor scenes and simulate Embodied AI tasks.

\subsection{Embodied AI tasks}
Basically, when we consider Embodied AI tasks in \framework, we decompose a task into elementary navigation and interaction tasks. The navigation task requires the agent to find and optimal route from one place to another while avoiding collisions. The interaction task often requires the agent to trigger the change of state of a certain object in the scene such as changing object location by the \textit{pickup} action.\framework  helps finishing navigation tasks and interaction tasks by providing the task-solving scripts to execute actions and examine whether a task is sucessfully completed.

\subsection{Language instructions}
Besides, \framework provides two methods to generate natural language descriptions along navigation and interaction tasks. The first method relies on a rule-based language template to generate language instructions for different tasks. The second method applies a transformer trained on \alfred\ annotations to generate language instructions from action sequences and video images.

\subsection{Basic usage}
As our framework contains different functions, we provide two generators, i.e., \textit{SceneGenerator}, \textit{TaskGenerator}, and
one solver \textit{TaskSolver} for users to manipulate \framework for different purposes. \textit{SceneGenerator} allows users to generated vary scenes from CDF files; \textit{TaskGenerator} helps design tasks that be executed in the scene; \textit{TaskSolver} helps embodied agent to solve a task and generates corresponeding action sequences, video images and natural language instructions.



==> article/introduction_v0.tex <==
\section{Introduction}

% Logic flow 

% Importance of indoor synthesis
% \GS{I edited this paragraph, please check} \lkxcom{resolved}
Indoor scene synthesis is widely used in many applications, including but not
limited to online virtual interior design~\cite{Planner5d}, home automation,
advertisement for furniture designs~\cite{IKEA}, and simulated
environments~\cite{kolve2017ai2} for training and evaluating embodied agents. 
Since indoor door scene synthesis is critical for many 
downstream tasks, it has seen a significant amount of
activity~\cite{yu2011make,fisher2012example,fisher2015activity,qi2018human,wang2019planit,luo2020end,zhou2019scenegraphnet}
from both the computer graphics and machine learning communities. Recently, with the
development of large-scale datasets and the impressive performance of deep
neural networks,
substantial progress~\cite{wang2019planit,wang2020sceneformer,luo2020end,zhang2020deep}
has been made in {\em automating} scene generation. However,  discrepancies in scene representation, datasets adopted, and rendering tools
present significant challenges in benchmarking performance and comparing scene generation techniques to each other. On the other hand, scene synthesis is a generative task that lacks ground truth for quantitative and automatic evaluation. The
predominant metrics such as bounding box and angle
prediction~\cite{luo2020end} and synthetic  classification~\cite{wang2019planit}
are not always positively correlated with the quality of the generated scene.
Towards resolving these issues, we propose \framework, a research framework for
indoor scene synthesis that provides unified evaluation protocol and rendering
tools. Further, we propose a set of complementary automatic evaluation
metrics based on the following principle: the ability to serve downstream tasks is the best measure of the quality of the synthesized scene. We first draw connections between embodied artificial intelligence (EAI) and indoor
scene synthesis, which naturally gives rise to our proposed metric. 

% Challenges in Embodied AI tasks. 
Embodied AI has attracted significant attention  due to the  development of simulated platforms~\cite{puig2018virtualhome,kolve2017ai2,gan2020threedworld}, computational power, and
advanced model architectures~\cite{vaswani2017attention,lu2019vilbert}. One
long-standing problem is the poor generalization of embodied agents, where we
typically observe a notable performance drop between seen and unseen environments~\cite{shridhar2020alfred,singh2020moca}. In addition to developing more
generalizable learning models, a promising direction is to improve the variety of simulated environments {e.g., domain 
randomization~\cite{shen2020igibson,kolve2017ai2}}.
% \GS{This sentence is unclear}
However, the layout of the environment in the previous approach remains unchanged. Similar to CoinRun~\cite{cobbe2019quantifying} that enhances the generalization of RL agent by procedurally generated environments, we propose
to generate indoor scenes that are readily available for learning embodied agents.
Unlike the current trend in Embodied AI that designs challenging tasks for learning agents to complete in a limited number of scenes, we seek a learning agent to accomplish simple tasks in various and a large number of environments. Furthermore,
the navigation, object interaction, task completion metric can, in turn 
serve as a reliable evaluation measurement for the generated scene. 


Our contribution is threefold. First, we introduce a unified research
framework (\framework) which serves as a standard and unified benchmark for indoor scene synthesis. Second, we connect the field of Embodied AI and scene synthesis
by proposing Embodied AI task to evaluate generated scene. Third, our framework can
generate an infinite number of scenes to facilitate generalization research for embodied agents.

% ---------------------------------------------------------------------------------


